LoFT: Local Proxy Fine-tuning For Improving Transferability Of Adversarial Attacks Against Large Language Model

It has been shown that Large Language Model (LLM) alignments can be circumvented by appending specially crafted attack suffixes with harmful queries to elicit harmful responses. To conduct attacks against private target models whose characterization is unknown, public models can be used as proxies to fashion the attack, with successful attacks being transferred from public proxies to private target models. The success rate of attack depends on how closely the proxy model approximates the private model. We hypothesize that for attacks to be transferrable, it is sufficient if the proxy can approximate the target model in the neighborhood of the harmful query. Therefore, in this paper, we propose \emph{Local Fine-Tuning (LoFT)}, \textit{i.e.}, fine-tuning proxy models on similar queries that lie in the lexico-semantic neighborhood of harmful queries to decrease the divergence between the proxy and target models. First, we demonstrate three approaches to prompt private target models to obtain similar queries given harmful queries. Next, we obtain data for local fine-tuning by eliciting responses from target models for the generated similar queries. Then, we optimize attack suffixes to generate attack prompts and evaluate the impact of our local fine-tuning on the attack's success rate. Experiments show that local fine-tuning of proxy models improves attack transferability and increases attack success rate by $39\%$, $7\%$, and $0.5\%$ (absolute) on target models ChatGPT, GPT-4, and Claude respectively.

==> figures/flow_diagram.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,252); %set diagram left start at 0, and has height of 252

%Shape: Rectangle [id:dp025237063148265793] 
\draw   (73.89,132.35) -- (189.11,132.35) -- (189.11,160.34) -- (73.89,160.34) -- cycle ;
%Shape: Rectangle [id:dp049988739083300926] 
\draw   (73.89,58.15) -- (189.11,58.15) -- (189.11,86.14) -- (73.89,86.14) -- cycle ;
%Straight Lines [id:da9262309830599416] 
\draw    (82.36,160.99) -- (82.36,173.61) ;
\draw [shift={(82.36,176.61)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da8203452411080966] 
\draw    (110.35,160.34) -- (110.35,172.96) ;
\draw [shift={(110.35,175.96)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da49545731436794205] 
\draw    (152,160.34) -- (152,172.96) ;
\draw [shift={(152,175.96)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da019488917991786647] 
\draw    (182.6,160.34) -- (182.6,172.96) ;
\draw [shift={(182.6,175.96)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da3387895136008259] 
\draw    (83.66,100.46) -- (96.68,86.14) ;
%Straight Lines [id:da6789309046836474] 
\draw    (110.35,100.46) -- (96.68,86.14) ;
%Straight Lines [id:da8158406429763265] 
\draw    (154.61,99.16) -- (168.28,86.79) ;
%Straight Lines [id:da4144638177138469] 
\draw    (181.29,99.81) -- (168.28,86.79) ;
%Straight Lines [id:da945579130400714] 
\draw    (81.71,117.38) -- (81.71,130) ;
\draw [shift={(81.71,133)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da02497180656416076] 
\draw    (109.69,116.73) -- (109.69,129.35) ;
\draw [shift={(109.69,132.35)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da5235556715686732] 
\draw    (151.35,116.73) -- (151.35,129.35) ;
\draw [shift={(151.35,132.35)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da7276467023493102] 
\draw    (181.95,116.73) -- (181.95,129.35) ;
\draw [shift={(181.95,132.35)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da3725261934142402] 
\draw    (94.07,42.53) -- (94.07,55.15) ;
\draw [shift={(94.07,58.15)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da6786600622210249] 
\draw    (168.28,42.53) -- (168.28,55.15) ;
\draw [shift={(168.28,58.15)}, rotate = 270] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Rectangle [id:dp48647262473613206] 
\draw   (234.51,50) -- (324,50) -- (324,144) -- (234.51,144) -- cycle ;
%Shape: Rectangle [id:dp3256540910925356] 
\draw   (339.86,158.75) -- (400,158.75) -- (400,190.75) -- (339.86,190.75) -- cycle ;
%Shape: Rectangle [id:dp6857958284863118] 
\draw   (346.81,79.23) -- (392.38,79.23) -- (392.38,118.94) -- (346.81,118.94) -- cycle ;
%Straight Lines [id:da8376104386116062] 
\draw    (324,99.76) -- (343.81,99.76) ;
\draw [shift={(346.81,99.76)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da3162479303629605] 
\draw    (369,158) -- (369,124.25) ;
\draw [shift={(369,121.25)}, rotate = 90] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Rectangle [id:dp5576229397553814] 
\draw   (413.21,79.89) -- (488,79.89) -- (488,119.59) -- (413.21,119.59) -- cycle ;
%Straight Lines [id:da09127931120805433] 
\draw    (393.03,100.41) -- (409.56,100.41) ;
\draw [shift={(412.56,100.41)}, rotate = 180] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Shape: Rectangle [id:dp3422058503399472] 
\draw   (528,63.5) -- (643,63.5) -- (643,130.25) -- (528,130.25) -- cycle ;
%Shape: Rectangle [id:dp7273429947515212] 
\draw   (528.89,167.19) -- (644.11,167.19) -- (644.11,195.18) -- (528.89,195.18) -- cycle ;
%Straight Lines [id:da06628387973325844] 
\draw    (583.5,46.75) -- (583.64,60.5) ;
\draw [shift={(583.67,63.5)}, rotate = 269.43] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;
%Straight Lines [id:da1504495639094907] 
\draw    (587,130.83) -- (586.85,164.25) ;
\draw [shift={(586.83,167.25)}, rotate = 270.26] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (10.72,-5.15) -- (0,0) -- (10.72,5.15) -- (7.12,0) -- cycle    ;

% Text Node
\draw (88.5,138.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{63pt}\setlength\topsep{0pt}
\begin{center}
{\large Target model}
\end{center}

\end{minipage}};
% Text Node
\draw (82.39,57.65) node [anchor=north west][inner sep=0.75pt, text height=0.45cm]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{69pt}\setlength\topsep{0pt}
\begin{center}
Generate LP from\\target model
\end{center}

\end{minipage}};
% Text Node
\draw (71.28,176.43) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle R_{1}^{1} \dotsc R_{1}^{M}$};
% Text Node
\draw (140.1,177.46) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle R_{K}^{1} \dotsc R_{K}^{M}$};
% Text Node
\draw (123.13,184.77) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle \dotsc $};
% Text Node
\draw (10.02,162.79) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\textbf{Similar}\\\textbf{query}\\\textbf{response}};
% Text Node
\draw (73.48,99.22) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle S_{1}^{1} \dotsc S_{1}^{M}$};
% Text Node
\draw (142.3,98.62) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle S_{K}^{M} \dotsc S_{K}^{M}$};
% Text Node
\draw (123.65,108.9) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle \dotsc $};
% Text Node
\draw (9.72,95.27) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\textbf{Similar}\\\textbf{query}};
% Text Node
\draw (85.1,22.72) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {$\displaystyle h_{1}$};
% Text Node
\draw (159.15,23.07) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {$\displaystyle h_{K}$};
% Text Node
\draw (9.26,22.99) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\textbf{Harmful}\\\textbf{query}};
% Text Node
\draw (236.51,45.5) node [anchor=north west][inner sep=0.75pt, text height=2.35cm]  [font=\normalsize] [align=left] {\textbf{Query:} $\displaystyle S_{1}^{1}$\\\textbf{Response:} $\displaystyle \mathcal{R}_{1}^{1}$\\$\displaystyle \ \ \ \vdots $\\\textbf{Query:} $\displaystyle S_{K}^{M}$\\\textbf{Response:} $\displaystyle \mathcal{R}_{K}^{M}$};
% Text Node
\draw (351.62,159.97) node [anchor=north west][inner sep=0.75pt, text height=0.45cm]  [font=\normalsize] [align=left] {\begin{minipage}[lt]{24.93pt}\setlength\topsep{0pt}
\begin{center}
Proxy\\model
\end{center}

\end{minipage}};
% Text Node
\draw (349.81,83.23) node [anchor=north west][inner sep=0.75pt, text height=0.48cm]  [font=\normalsize] [align=left] {\begin{minipage}[lt]{30pt}\setlength\topsep{0pt}
\begin{center}
Fine-\\tuning
\end{center}

\end{minipage}};
% Text Node
\draw (422.81,85.56) node [anchor=north west][inner sep=0.75pt, text height=0.4cm]  [font=\normalsize] [align=center] {\begin{minipage}[lt]{39pt}\setlength\topsep{0pt}
\begin{center}
Local\\FT model%
\end{center}
\end{minipage}};
% Text Node
\draw (23.17,218.5) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\textbf{1. Local Prompt (LP) generation}};
% Text Node
\draw (320,219) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\textbf{2. Local fine-tuning}};
% Text Node
\draw (549.5,25.5) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {Attack query};
% Text Node
\draw (533.68,68.5) node [anchor=north west][inner sep=0.75pt, text height=0.8cm] [font=\normalsize]  [align=left] {\begin{minipage}[lt]{76pt}\setlength\topsep{0pt}
\begin{center}
Attack algorithm\\on\\Local FT model
\end{center}

\end{minipage}};
% Text Node
\draw (590.83,139.5) node [anchor=north west][inner sep=0.75pt]  [font=\normalsize] [align=left] {Attack response};
% Text Node
\draw (533,172.33) node [anchor=north west][inner sep=0.75pt, text height=0.3cm]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{78pt}\setlength\topsep{0pt}
\begin{center}
{\large $\displaystyle \star $Target model}
\end{center}

\end{minipage}};
% Text Node
\draw (529.5,217.5) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {\textbf{3. Attack evaluation}};
% Text Node
\draw (120.65,29.9) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle \dotsc $};


\end{tikzpicture}

